FPT Approximations for Packing and Covering Problems Parameterized by Elimination Distance and Even Less

For numerous graph problems in the realm of parameterized algorithms, using the size of a smallest deletion set (called a modulator) into well-understood graph families as parameterization has led to a long and successful line of research. Recently, however, there has been an extensive study of structural parameters that are potentially much smaller than the modulator size. In particular, recent papers [Jansen et al. STOC 2021; Agrawal et al. SODA 2022] have studied parameterization by the size of the modulator to a graph family $\mathcal{H}$ ($\textbf{mod}_{\mathcal{H}}$), elimination distance to $\mathcal{H}$ ($\textbf{ed}_{\mathcal{H}}$), and $\mathcal{H}$-treewidth ($\textbf{tw}_{\mathcal{H}}$). While these new parameters have been successfully exploited to design fast exact algorithms their utility (especially that of latter two) in the context of approximation algorithms is mostly unexplored. The conceptual contribution of this paper is to present novel algorithmic meta-theorems that expand the impact of these structural parameters to the area of FPT Approximation, mirroring their utility in the design of exact FPT algorithms. Precisely, we show that if a covering or packing problem is definable in Monadic Second Order Logic and has a property called Finite Integer Index, then the existence of an FPT Approximation Scheme (FPT-AS, i.e., ($1\pm \epsilon$)-approximation) parameterized these three parameters is in fact equivalent. As concrete exemplifications of our meta-theorems, we obtain FPT-ASes for well-studied graph problems such as Vertex Cover, Feedback Vertex Set, Cycle Packing and Dominating Set, parameterized by these three parameters.

==> PreambleNew.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\iffalse
%\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}

\usepackage{mdframed}
\usepackage{tcolorbox}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}
\usepackage{tcolorbox}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}
\fi 

\newtheorem{theorem}{Theorem}[section]
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}[lemma]{Claim}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{observation}[lemma]{Observation}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{redrule}[lemma]{Reduction Rule}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{reduction}[lemma]{Reduction Rule}
\newtheorem{conjecture}[lemma]{Conjecture}

\date{}
 
%\newcommand{\defparproblem}[4]{
%\vspace{1mm}
%\noindent\fbox{
%  \begin{minipage}{0.96\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
%  {\bf{Input:}} #2  \\
%  {\bf{Question:}} #4
%  \end{minipage}
%}\vspace{1mm}}
%
%\newcommand{\defproblem}[3]{
%\vspace{1mm}
%\noindent\fbox{
%  \begin{minipage}{0.96\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
%  {\bf{Input:}} #2  \\
%  {\bf{Question:}} #3
%  \end{minipage}
%}\vspace{1mm}}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usetikzlibrary{decorations.markings}

  \tikzset{vo/.style = {
		shape= circle,
		fill = blue,
		inner sep = 2pt,
		outer sep = 0pt,
		minimum size = 8 pt}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\OO}{\mathcal{O}}
%\newcommand{\cS}{\mathcal{S}}
\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
%\newcommand{\tw}{\mathtt{tw}}
%\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\textsf{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\domain}{\mbox{\sf dom}}
\newcommand{\image}{\mbox{\sf ima}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}
								
% Paper-specific commands								
\newcommand{\Mark}{\textsf{Mark}}
\newcommand{\mar}{\mbox{\sf mark}}
\newcommand{\vis}{\mbox{\sf vis}}

\newcommand{\cSuccessEnough}{$2$}
\newcommand{\cSuccessStage}{$1$}
\newcommand{\cBigClique}{$10$}
\newcommand{\cHeavyMark}{$3$}
\newcommand{\cVisibleOut}{$1$}
\newcommand{\cVisibleIn}{$1$}

\newcommand{\sm}{\setminus}
%\newcommand{\kk}{{k^{1/2}}}
\newcommand{\kk}{{\sqrt{k}}}
\newcommand{\kkk}{{k^{3/2}}}

\newcommand{\hy}{\widehat{Y}}
\newcommand{\hx}{\widehat{X}}
\newcommand{\hc}{\widehat{C}}
\newcommand{\hs}{\widehat{S}}
\newcommand{\ha}{\widehat{A}}
\newcommand{\la}{\leftarrow}

%% Problem Names 
\newcommand{\vcfull}{{\sc Vertex Cover}\xspace}
\newcommand{\fvstfull}{{\sc Feedback Vertex Set in Tournaments}\xspace}
\newcommand{\fvst}{{\sc FVST}\xspace}
\newcommand{\fvsfull}{{\sc Feedback Vertex Set}\xspace}
\newcommand{\fvs}{{\sc FVS}\xspace}

\newcommand{\dspfull}[1]{$#1$-\text{{\sc Set Packing}}\xspace}
\newcommand{\ddmfull}[1]{$#1$-\text{{\sc Dimensional Matching}}\xspace}
\newcommand{\dhsfull}[1]{$#1$-\text{{\sc Hitting Set}}\xspace}

\newcommand{\dhs}[1]{$#1$-\text{{\sc HS}}\xspace}
\newcommand{\hsetfull}{{\sc Hitting Set}\xspace}
\newcommand{\hset}{{\sc HS}\xspace}


\newcommand{\cvdfull}{{\sc Cluster Vertex Deletion}\xspace}
\newcommand{\cvd}{{\sc CVD}\xspace}

\newcommand{\ippfull}{{\sc Induced $P_3$-Packing}\xspace}
\newcommand{\tptfull}{{\sc Triangle Packing in Tournaments}\xspace}
\newcommand{\tpt}{{\sc TPT}\xspace}

\DeclareMathOperator{\poly}{poly}
\newcommand{\good}{output-parameter sensitive}

==> maintheorem-cvc.tex <==

\subsection{Equivalence Theorem for Connected Vertex Cover and Connected Dominating Set} \label{subsec:equivalence-cvc}

\todo[inline]{discuss modification to domset theorem}

==> mainthorem.tex <==
%!TEX root = main.tex

\iffalse
\section{Results} 




\begin{itemize}
\item  Equivalences with FPT approximation schemes parameterized by $mod_H$,  $elmn_H$. and  $tw_H$. 
A problem $\Pi$ admits FPT approximation parameterized by $mod_H \iff elmn_H \iff tw_H$. 
Example: {\sc Vertex Cover} parameterized by planar deletion set. 

This requires notion of generalized lossless protrusion replacer. 

\item Individual Pieces to plug into this main result. This includes treewidth$\eta$deletion param by something. 

\item Bucket and ocean scheme also gives lossy kernels. 

\item Maximization problems -- {\sc Independent Set}, {\sc Planar $F$-Packing} and {\sc Cycle Packing}   same strategy 

\item {\sc Dominating Set} 
\item Lossy Turing Kernels

\end{itemize}
\fi








==> modulator-results.tex <==
%!TEX root = main.tex

\section{FPT-AS Parameterized by \texorpdfstring{$\mdh(G)$}{mod\_H(G)}}
\iffalse








\iffalse By iterating over all possibilities, we ``guess'' the intersection of an optimal (usual) dominating set $S^*$ for $G$ with the modulator $X$. Consider a fixed guess $Y \subseteq X$, and let $U \coloneqq X \setminus Y$. In the current iteration, our aim is to compute a candidate dominating set for $G$ that contains \emph{all} vertices from $Y$. In the end, we will return the minimum-size candidate solution found over all iterations.

Let $H \coloneqq V(G) \setminus X$, and let $D = N(Y) \cap H$. Note that $G' = G[H] \in \cH$. Let $(G', D)$ denote the resulting instance of annotated dominating set, where all the vertices of $D$ are marked as dominated. Since $G' \in \cH$, we use the EPTAS from Fomin et al.\ \cite{FominLS18Grid} to obtain a solution $S' \subseteq H$ such that $|S'| \le (1+\frac{\epsilon}{2}) \cdot \OPT(G', D)$ in time $2^{\Oh(1/\epsilon)} \cdot \polyn$. Now, we consider two cases similar to the previous section.

\paragraph{Case 1.} $p \le \frac{\epsilon}{3} \cdot |S'|$.
\\In this case, we return $X \cup S'$ as a candidate solution in this iteration. We have the following claim.
\begin{claim} \label{cl:domset-case1}
	Let $S^* \subseteq V(G)$ be an optimal dominating set for $G$, and suppose the solution $S'$ found in the iteration corresponding to $Y^* \coloneqq S^* \cap X$ satisfies the condition for Case 1, i.e., $p \le \frac{\epsilon}{3} \cdot |S'|$. Then, $|X \cup S'| \le (1+\epsilon) \cdot |S^*|$.
\end{claim}
\begin{proof}
	Consider the iteration corresponding to $Y = Y^*$, and consider the corresponding instance $(G', D^*)$ of the annotated dominating set as previously defined. Note that since $Y^* \subseteq S^*$, all vertices of $D^* = N(Y^*) \cap H$ are dominated by $Y^*$. 
	
	Now consider any vertex $u \in H \setminus D^*$. Either $u \in S^*$, or some $v \in N(u)$ must belong to $S^*$. Now, we prove that that $v \in H$. Suppose for the contradiction that $v \in X$. Then, $v \in X \cap S^* = Y^*$. However, this implies that $u \in D$, which is a contradiction. Thus, $S^* \setminus Y^*$ is a dominating set for all the vertices in $H \setminus D^*$, i.e., $S^* \setminus Y^*$ is a feasible solution for the annotated instance $(G', D^*)$ \footnote{Note that $S^* \setminus Y^*$ may not be an optimal solution for the annotated instance $(G', D^*)$, since it may also contain additional vertices in order to dominate the vertices in $X \setminus Y^*$, which is not a requirement for the annotated instance.}. Therefore, using Case 1 assumption, we get the following.
	\begin{align*}
		|X| + |S'| \le (1 + \frac{\epsilon}{3}) \cdot |S'| &\le (1+\epsilon) \cdot \OPT(G', D^*) 
		\\&\le (1+\epsilon) \cdot |S^* \setminus Y| \tag{Since $S^* \setminus Y$ is a feasible solution for $(G', D^*)$}
		\\&\le (1+\epsilon) \cdot |S^*|
	\end{align*}
\end{proof}

\paragraph{Case 2.} $p > \frac{\epsilon}{3} |S'|$, i.e., $\OPT(G', D) \le |S'| < \frac{3p}{\epsilon}$.

We design an exact FPT algorithm parameterized by the solution size in this case. First, note that \Cref{lem:contraction-bidim} and \Cref{prop:sqgc} imply that $\tw(G') \le \sqrt{OPT(G', D)} = \Oh(\sqrt{p/\epsilon})$. From here, we observe that $\tw(G) \le \tw(G') + |X| \le \Oh(\sqrt{p/\epsilon}) + p$. In this case, we simply use a single-exponential \FPT algorithm for \domset parameterized by treewidth. Thus, we have the following claim.

\begin{claim} \label{cl:domset-case2}
	%Let $S^* \subseteq V(G)$ be an optimal dominating set for $G$, and suppose the solution $S'$ found in the iteration corresponding to $Y^* \coloneqq S^* \cap X$ satisfies the condition for Case 1, i.e., $p \le \frac{\epsilon}{3} \cdot |S'|$. 
	Suppose in any iteration, the condition corresponding to Case 2 is satisfied. Then, we can find an optimal solution to \domset on $G$ in time $2^{\Oh(p + \sqrt{p/\epsilon})} \cdot \polyn$.
\end{claim}

By combining the results corresponding to the two cases, we obtain the following theorem.

\begin{theorem}
	Suppose we are given a graph $G = (V, E)$, and a set $X \subseteq V(G)$ of size $p$, such that $G' \coloneqq G \setminus X \in \cH$. Then, there exists an $2^{\Oh(p + \frac{1}{\epsilon} + \sqrt{\frac{p}{\epsilon}})} \cdot \polyn$ time algorithm to find a $(1+\epsilon)$-approximation for \domset on $G$.
\end{theorem}


Let $R \coloneqq V(G) \setminus X$. Since we add all vertices of $Y$ to the solution, all vertices from $N(Y)$ will be dominated. We mark this by coloring them \emph{red}, and refer to such a vertex as a \emph{dominated} vertex. If a vertex is neither dominated, nor belongs to $Y$, then it is said to be \emph{undominated}. If some vertex from $U$ is dominated, we remove it from consideration in this guess. On the other hand, if there exists a vertex $u \in U$, such that $N(u) \subseteq U$, then clearly there cannot exist a dominating set $S$ with the aforementioned properties. In this case, we terminate this iteration, and proceed to the next guess $Y$. Thus, wlog we may assume that every $u \in U$ is undominated, and contains a neighbor outside $X$. 
\fi

\subsection{FPT-AS for Connected Vertex Cover par by $\mdh(G)$}
We are given a graph $G$ with a modulator $M$ to a family of graphs that excludes some fixed apex graph $H$ as a minor. Given an $\epsilon >0$, we fix an $\epsilon'=\frac{\epsilon}{5}$. Our objective is to find a connected vertex cover $S \subseteq V(G)$ of $G$ of size $|S| \leq (1 + \epsilon) \ \OPT_{CVC}(G)$ where $\OPT_{CVC}(G)$ denotes the size of the optimum connected vertex cover of $G$. Recall that a vertex set $S \subseteq V(G)$ is called connected vertex cover if $S$ is a vertex cover of $G$ and $G[S]$ is connected. {\color{Red}We can assume that the graph has no isolated vertices as we can safely remove those as those are not part of any optimum solution}. We will essentially use our favorite "bucket vs ocean" trick. We start with some known results that will eventually be used in our algorithm.

\begin{lemma}
	\label{lem:exact}
	For a given graph $G$ and a fixed integer $k \geq 0$, we can find a connected vertex cover of $G$ of size at most $k$ in time $f(k). n^{\mathcal{O}(1)}$ for some computable function $f$.{\color{Red}(need to add references)}
\end{lemma}
%Our algorithm has two phases

Observe that connected vertex cover is such a structural property of a graph which is not necessarily preserved when restricted to it's induced subgraphs. More elaborately, for a given connected graph $G$, if $G$ has a connected vertex cover $S$, then for any induced subgraph $G[Y]$ of $G$, $(S \cap Y)$ is a vertex cover but not necessarily a connected vertex cover for $G[Y]$. On top of that, $(S \cap Y)$ has a special property that every connected component of it {\em sees} a vertex of $M$. This leads us to an another variant of vertex cover problem which will be used later in our algorithm and stated below:\\

\begin{tcolorbox}[colback=white!5!white,colframe=gray!75!black]
	\xvc
	\\\textbf{Input:} A graph $G'$, a set $X \subseteq V(G)$
	\\\textbf{Objective:} Find a minimum vertex cover of $G'$ such that every connected component of contains a vertex from $X$?
\end{tcolorbox}

\begin{lemma}
	\label{lem:xvc}
	For any fixed $\epsilon'> 0$, there exist an algorithm for $\xvc$ which outputs a vertex cover $S$ of size $|S| \leq (1 + \epsilon') \OPT_{X-VC}(G')$ where $\OPT_{X-VC}(G')$ is a optimum vertex cover for $\xvc$ and we can compute it in time .......
\end{lemma}

Recall that our original connected vertex cover problem has input as $G$ and $M$. First we want to solve $\xvc$ problem in the graph $G \setminus M$. In order to do that, we put $G'= G \setminus M$ and $X = N(M)$ and using Lemma~\ref{lem:xvc}, we compute a solution $\xvc$, $S'$ of size $(1 + \epsilon') \OPT_{X-VC}(G')$. Next we prove some useful lemmas

\begin{lemma}
	$\OPT_{X-VC}(G') \leq \OPT_{CVC}(G)$
\end{lemma}

\begin{proof}
	Let $Y$ be an optimum solution for connected vertex cover problem in $G$. Hence, $|Y| =  \OPT_{CVC}(G)$. Recall that $G' = G \setminus M$ and $X = N(M)$. Observe that, every connected component of $Y \cap G'$ has a neighbour in $M$. So, $Y \cap G'$ is a feasible solution for $\xvc$ of $G'$. Hence, $\OPT_{X-VC}(G') \leq |Y \cap G'| \leq |Y| = \OPT_{CVC}(G)$. This concludes the proof of the lemma.
\end{proof}

\begin{lemma}
	\label{lem:makeconnected}
	For a given solution $S''$ to $\xvc$ in $G'$, we can construct a connected vertex cover of $G$ of size at most $(|S''| +2|M|)$ in $n^{\mathcal{O}(1)}$ time.
\end{lemma}

\begin{proof}
	Notice that $(S'' \cup M)$ is a vertex cover of $G$ but might not be a connected vertex cover of $G$. If $G[S''\cup M]$ is connected, we are done. Otherwise, for every two connected component in $G[S''\cup M]$, $G'\setminus S''$ has a vertex which is neighbor to both of them. Add that vertex to $(S'' \cup M)$. Observe that every such addition reduces the number of connected component of $(S'' \cup M)$. Since $G[S'' \cup M]$ has at most $|M|$ connected components, we need to repeat this procedure at most $(|M| -1)$ times to make it connected. At the end, the size of the connected vertex cover solution will be at most $(|S''| +2|M| - 1)$. The whole process takes polynomial time which concludes the proof.
\end{proof}

\begin{lemma}
	\label{lem:connectedvc}
	$\OPT_{CVC}(G) \leq \OPT_{X-VC}(G') + 2|M|$
\end{lemma}

\begin{proof}
	Let $Z$ be an optimum solution for the problem $\xvc$ in $G'$. Hence, $|Z| = \OPT_{X-VC}(G')$. Using Lemma~\ref{lem:makeconnected}, we construct a feasible solution of connected vertex cover problem of size at most $(\OPT_{X-VC}(G') + 2|M|)$. Hence, $\OPT_{CVC}(G) \leq \OPT_{X-VC}(G') + 2|M|$ which concludes the proof.
\end{proof}

After getting $S'$, we compare the size of $S'$ with the size of the modulator $M$ and accordingly we divide it into two cases.

\begin{itemize}
	\item Case 1: $|M| > \epsilon'|S'|$, implies that $|S'| < |M|/ \epsilon'$. That means size of the approximate solution $S'$ for $\xvc$ in $G'$ is upper bounded by $f(|M|, \epsilon')$ for some computable function $f$. Which implies that $\OPT_{X-VC}(G') \leq |S'| \leq |M|/ \epsilon'$. Further, using Lemma~\ref{lem:connectedvc}, we can say that $\OPT_{CVC}(G) \leq \OPT_{X-VC}(G') + 2|M|$ which implies that $\OPT_{CVC}(G)$ is upper bounded by $g(|M|, \epsilon')$ for some computable function $g$. Further using Lemma~\ref{lem:exact}, we plug in the value of $k$ to be  $g(|M|, \epsilon')$ and compute a connected vertex cover $S$ in FPT time parameterized by modulator and $\epsilon'$ . Hence, in this case, we solve our problem exactly.
	
	\item Case 2: $|M| \leq \epsilon'|S'|$. Starting from $S'$, using Lemma~\ref{lem:makeconnected}, we construct a connected vertex cover $S = (S'\cup M \cup M^{\ast})$ of size at most $|S' \cup M \cup M^{\ast}| \leq (|S'| + |M| + |M^{\ast}|) \leq(|S'| + 2|M|) \leq (1 + 2 \epsilon')|S'| \leq (1 + 2 \epsilon')(1 + \epsilon')\OPT_{CVC}(G) = (1 + 3 \epsilon' + 2\epsilon'^2) \OPT_{CVC}(G) \leq (1 + 5 \epsilon')\OPT_{CVC}(G) = (1 + \epsilon)\OPT_{CVC}(G)$. Hence, in this case, we get an $(1 + \epsilon)$ approximate solution.
	
	
	
	%is a subset of $X= N(M)$ of size 
	%\begin{claim}
	%	$S$ is a connected vertex cover of $G$.
	%\end{claim}
	%\begin{proof}
	%	First notice that, using Lemma~\ref{lem:xvc}  $S'$ is a vertex cover for $G'$ of size $|S'| \leq (1 + \epsilon')\OPT_{X-VC}$,
	%\end{proof}
	
	
\end{itemize}























==> preliminariesOLD.tex <==
%!TEX root = main.tex
\section{Preliminaries}

For an instance $\cI$ of an optimization problem $\Pi$, we denote the value/size of an optimal solution by $\OPT_\Pi(\cI)$, and may omit the subscript if the problem is clear from the context. An algorithm that, for any feasible instance of minimization (resp.\ maximization) problem $\Pi$, returns a solution of cost/size at most (resp.\ at least) $\alpha \cdot \OPT$, is called an $\alpha$-approximation. We say that a minimization (resp.\ maximization) problem $\Pi$ admits an \FPTAS (FPT-Approximation Scheme) parameterized by a parameter $t$ and $\epsilon$, if there exists an $(1+\epsilon)$-approximation (resp.\ $(1-\epsilon)$-approximation) algorithm with running time of the form $f(t, \epsilon) \cdot |\cI|^{\Oh(1)}$, for some computable function $f$. Similarly, we say that $\Pi$ admits an \EPTAS (efficient polynomial-time approximation scheme), if there exists an $(1+\epsilon)$-approximation (resp.\ $(1-\epsilon)$-approximation) algorithm with running time of the form $g(\epsilon) \cdot |\cI|^{\Oh(1)}$, for some computable function $g$.

\todo[inline]{Basics on graphs: vertex deletion, subgraphs, minors, disjoint unions.}

\begin{definition}[Graph Minor]
	A graph $H$ is a \emph{minor} of $G$ if it can be obtained by a sequence of vertex deletions, edge deletions, and edge contractions.
\end{definition}


Let $\cG$ denote the family of all graphs. We say that a family $\cF \subseteq \cG$ of graphs is \emph{hereditary} if for any graph $G \in \cF$, every induced subgraph $G'$ of $G$ also belongs to $\cF$. We say that a family $\cF \subseteq \cG$ is \emph{closed under disjoint union} if for any $G_1, G_2 \in \cF$, the graph $G$ obtained by taking the disjoint union of $G_1$ and $G_2$, also belongs to $\cF$. We say that a family $\cF \subseteq \cG$ is \emph{well-behaved} if it is (i) hereditary, and (ii) closed under disjoint union. 

\todo[inline]{Tree decompositions, treewidth, modulator, elimination distance, treewidth wrt $\cH$.}

The following definitions are borrowed from \cite{AgrawalKLPRSZ22Elimination}.

\begin{definition} \label{def:h-elimination-decomp}
	For a graph family $\cH$, an \emph{$\cH$-elimination decomposition} of $G$ is a triple $(T, \chi, L)$, where $T$ is a rooted forest, $\chi: V(T) \to 2^{V(G)}$, and $L \subseteq V(G)$ such that:
	\begin{enumerate}
		\item For each internal node $t \in V(T)$, we have that $|\chi(t)| \le 1$, and $\chi(t) \subseteq V(G) \setminus L$.
		\item The sets $(\chi(t))_{t \in V(T)}$ form a partition of $V(G)$.
		\item For each leaf $t$ in $T$, we have $\chi(t) \subseteq L$, such that the graph $G[\chi(t)]$, called a base component, belongs to $\cH$. Furthermore, $(\chi(t))_{\text{leaf} t}$ forms a partition of $L$.
		\item For each edge $uv \in V(G)$, if $u \in \chi(t_1)$, and $v \in \chi(t_2)$, then $t_1$ and $t_2$ are in ancestor-descendant relation in $T$.
	\end{enumerate}
\end{definition}

The depth of a rooted tree $T$ is the maximum number of edges on a root-to-leaf path in $T$. We refer to the union of base components as the set of base vertices. The $\cH$-elimination distance of $G$, denoted as $\edh(G)$, is the minimum depth of an $\cH$-elimination forest for $G$. Note that a pair $(T, \chi)$ is a (standard) elimination forest of $\cH$ is a class of empty graphs, i.e., the base components are empty. In this case, $\edh(G)$ is known as the \emph{treedepth} of $G$, and is denoted as $\td(G)$.

Just like the notion of $\cH$-elimination decomposition generalizes the notion of elimination forest, the following is an analogous generalization of the notion of tree decomposition.

\begin{definition} \label{def:h-treewidth}
	For a graph family $\cH$, an \emph{$\cH$-tree decomposition} of a graph $G$ is a triple $(T, \chi, L)$, where $T$ is a rooted tree, $\chi: V(T) \to 2^{V(G)}$, and $L \subseteq V(G)$, such that:
	\begin{enumerate}
		\item For each $v \in V(G)$, the nodes $\LR{t \in V(T) : v \in \chi(t)}$ induce a non-empty connected subtree in $T$.
		\item For each edge $uv \in E(G)$, there is a node $t \in V(G)$ with $\{u, v\} \in \chi(t)$.
		\item For each vertex $v \in L$, there is a \emph{unique leaf} $t \in V(T)$ for which $v \in \chi(t)$. 
		\item For each node $t \in V(T)$, the graph $G[\chi(t) \cap L] \in \cH$.
	\end{enumerate}
\end{definition}

The \emph{width} of an $\cH$-tree decomposition is defined as $\max\LR{ 0, \max_{t \in V(T)} |\chi(t) \setminus L| - 1 }$. The $\cH$-treewidth of $G$, denoted by $\twh(G)$, is the minimum width of an $\cH$-tree decomposition of $G$. The connected components of $G[L]$ are called base components, and the vertices in $L$ are called base vertices. 

A pair $(T, \chi)$ is a (standard) \emph{tree decomposition} if $(T, \chi, \emptyset)$ satisfies all conditions of an $\cH$-decomposition, where the choice of $\cH$ is irrelevant. 


